GenShare: Sharing Accurate Differentially-Private Statistics for Genomic Datasets with Dependent Tuples

Motivation: Cutting the cost of DNA sequencing technology led to a quantum leap in the availability of genomic data. While sharing genomic data across researchers is an essential driver of advances in health and biomedical research, the sharing process is often infeasible due to data privacy concerns. Differential privacy is one of the rigorous mechanisms utilized to facilitate the sharing of aggregate statistics from genomic datasets without disclosing any private individual-level data. However, differential privacy can still divulge sensitive information about the dataset participants due to the correlation between dataset tuples. Results: Here, we propose GenShare model built upon Laplace-perturbation-mechanism-based DP to introduce a privacy-preserving query-answering sharing model for statistical genomic datasets that include dependency due to the inherent correlations between genomes of individuals (i.e., family ties). We demonstrate our privacy improvement over the state-of-the-art approaches for a range of practical queries including cohort discovery, minor allele frequency, and chi^2 association tests. With a fine-grained analysis of sensitivity in the Laplace perturbation mechanism and considering joint distributions, GenShare results near-achieve the formal privacy guarantees permitted by the theory of differential privacy as the queries that computed over independent tuples (only up to 6% differences). GenShare ensures that query results are as accurate as theoretically guaranteed by differential privacy. For empowering the advances in different scientific and medical research areas, GenShare presents a path toward an interactive genomic data sharing system when the datasets include participants with familial relationships.

==> 7-TableOfContents.tex <==
\begin{table}[H]
\centering
\processtable{Table of notations\label{Tab:01}} {\begin{tabular}{p{15mm} | p{7cm}}\toprule \\ Notation&Explanation\\\midrule
$\textit{A}$ & A mechanism produces outputs with noise drawn from a suitable Laplace distribution. \\
$Range($\textit{A}$)$ & The domain of the output under mechanism $\textit{A}$, $\textit{O}$ $\in$ $Range($\textit{A}$)$\\
$\textit{Q}$ & The Query function \\
$\epsilon$ & Parameter expressing the privacy budget \\
$\textit{D}$ & The actual dataset \\
$\textit{${D}'$}$ & Neighboring dataset \\
$\textit{S}$ & The set of SNPs IDs \\
$\textit{m}$ & The number of SNPs \\
$\textit{i}$ & A SNP in $\textit{S}$ \\
$\textit{n}$ & Number of participants in the dataset \\
%$\textit{k}$ & The SNP value, k\in\{0,1,2\} \\
$\textit{X}$ & An m$\times$n matrix that stores the values of the SNPs for all members\\
$\textit{$X_{j}$}$ & The set of SNPs for an individual $\textit{j}$\\
$\mathbf{B}$ & The set of correlated participants in the dataset, $|\mathbf{B}|$ = b\\
$\textit{$j$}$  & A targeted participant in the dataset ($j$ in $\mathbf{B})$ \\

$\psi$ & The dependent participants with the target $j$ in the dataset ($\psi$ = $\mathbf{B} \setminus j$)$ \\
$\textit{$k$}$  & A family member participated in the dataset ($k$ in $\mathbf{\psi})$ \\
$\textit{$o$}$  & A family member participated in the dataset ($o$ in $\mathbf{\psi})$ \\
$\textit{h}$ & The SNP value for a tuple $j$ in $\textit{D}$ \\
$\textit{h'}$ & The SNP value for a tuple $j$ in $\textit{D'}$ (h' holds the value that gives maximum change with $\textit{h}$ (e.g. if $\textit{h}$ = 2 then $\textit{h'}$ = 0)\\
$\tilde{h}$ & A sanitized SNP value for a tuple $\textit{h}$ in $\textit{D}$ \\
$\textit{a}$ & The SNP value for tuples $\psi$ in $\textit{D}$ a\in\{0,1,2\} \\
$\bar{a}$ &  \\
$\mathbb{A}$ &  \\
%the genomic records of target j %actual (correct) SNP set $X_{j}$
%$\textit{$\tilde{D_{pj}^{i}}$}$ & The noisy query results\\
$\Delta Q$ & The global sensitivity of the query\\
$\sigma$ & The added noise due to tuples correlation \\
$\varsigma$ & Our new dependent sensitivity $\varsigma = \Delta Q + \sigma$ \\
$\lambda$ & Laplace distribution scale $\lambda = (\Delta Q / \epsilon)\\
$\textit{$x_{i}^{j}$}$ & The SNP value $\textit{i}$ for individual $\textit{$j$}$\\
$\tilde{$x_{i}^{j}$}$ & The estimated SNP value $\textit{i}$ for individual $\textit{$j$}$\\
$\textBf{$X_{i}^{\psi}$}$ & The set of SNP $\textit{i}$ values for dependent individuals in $\textit{$\psi$}$ (|X_{i}^{\psi}| = \psi)\\
$\tilde{$X_{i}^{\psi}$}$ & The estimated SNP value $\textit{i}$ for individual $\textit{$j$}$\\
%$\textit{d}$ & The size of the tuples which are correlated with the individual $\textit{j}$\\

\end{tabular}}{} 
\end{table}.

